The ALMA Survey of Gas Evolution of PROtoplanetary Disks (AGE-PRO): Formaldehyde (H$_2$CO) emission and its links to disk properties

Protoplanetary disks are rotating structures of gas and dust surrounding young stars, serving as the birth places of planets. Understanding the chemical evolution of organic materials in these disks is key for tracing the origins of organics in planetary systems. Formaldehyde (H$_2$CO) is the most commonly detected organic molecule in protoplanetary disks. In this study, we investigate the emission of H$_2$CO and its link to disk properties, using a sample of 20 Class II disks in the Lupus and Upper Sco star-forming regions spanning over 1-6 Myr. We analyze the H$_2$CO lines at 218.222 and 290.623 GHz observed as part of the AGE-PRO ALMA Large Program. Within this sample we achieve a detection rate of H$_2$CO of 45% (9/20), and set robust upper limits for the non-detections. We measure the excitation temperature and column density of the H$_2$CO gas in the sources with H$_2$CO detections. We combine our sample with 13 additional disks with archival H$_2$CO detections and search for correlations between H$_2$CO properties and disk parameters. Notably, we find strong correlations between H$_2$CO line luminosity and dust radius, gas radius, dust mass, gas mass, stellar mass, and stellar luminosity. This suggests that H$_2$CO emission is brighter for extended massive dust disks where H$_2$CO can form via CO ice hydrogenation on grain surfaces. We find that the H$_2$CO excitation temperature is also correlated with stellar mass and stellar luminosity, so more massive and luminous stars could increase H$_2$CO excitation.

==> obs_log.tex <==
\begin{deluxetable*}{lllllllll}
\tabletypesize{\scriptsize}
\tablecaption{AGE-PRO Observational log \label{table:obs_log}}
\tablewidth{0pt}
\tablehead{
\colhead{Setup} & \colhead{Source Name} & \colhead{UTC Date} & \colhead{Config}  & \colhead{Baselines} & 
\colhead{N$_{\rm ant}$} & \colhead{Elev} & \colhead{PWV} & \colhead{Calibrators} 
\\
\colhead{} & \colhead{} &  \colhead{} & \colhead{} & \colhead{(m)} & 
\colhead{} & \colhead{(deg)} & \colhead{(mm)} & \colhead{}
}
\decimalcolnumbers
\startdata
 Oph CO         &  Oph 1-6, 8-10            &  2022-03-29 06:06:   &  C43-2  &  14.6 - 313.7   &     45&   65.3&    2.2&  J1517-2422, J1625-2527   \\
  &  Oph 1-6, 8-10            &  2022-03-30 06:34:   &  C43-2  &  14.6 - 313.7   &     45&   72.5&    1.1&  J1517-2422, J1625-2527   \\
  &  Oph 1-6, 8-10            &  2022-04-08 05:35:   &  C43-2  &  14.6 - 313.7   &     45&   67.2&    0.5&  J1517-2422, J1625-2527   \\
  &  Oph 1-6, 8-10            &  2022-07-03 03:10:   &  C43-5  &  15.3 - 1301.6  &     42&   67.4&    0.5&  J1517-2422, J1700-2610   \\
  &  Oph 1-6, 8-10            &  2022-07-05 02:17:   &  C43-5  &  15.1 - 1996.7  &     41&   76.6&    1.5&  J1517-2422, J1700-2610   \\
  &  Oph 1-6, 8-10            &  2022-07-05 03:50:   &  C43-5  &  15.1 - 1996.7  &     41&   55.8&    1.5&  J1517-2422, J1700-2610   \\
  &  Oph 1-6, 8-10            &  2022-07-16 21:35:   &  C43-6  &  15.1 - 2617.4  &     42&   49.2&    0.7&  J1517-2422, J1700-2610   \\
  &  Oph 1-6, 8-10            &  2022-07-16 22:59:   &  C43-6  &  15.1 - 2617.4  &     41&   68.3&    0.6&  J1517-2422, J1700-2610   \\
  &  Oph 1-6, 8-10            &  2022-07-18 01:32:   &  C43-6  &  15.3 - 2617.4  &     44&   75.4&    0.5&  J1517-2422, J1700-2610   \\
  &  Oph 1-6, 8-10            &  2022-07-18 23:10:   &  C43-6  &  15.3 - 2617.4  &     43&   71.8&    1.4&  J1517-2422, J1700-2610   \\
 Oph C$^{17}$O  &  Oph 1-10                 &  2022-04-03 11:09:   &  C43-2  &  14.6 - 360.6   &     44&   40.8&    1.3&  J1924-2914, J1700-2610   \\
  &  Oph 1-10                 &  2022-04-09 05:31:   &  C43-2  &  15.0 - 313.7   &     41&   67.0&    0.9&  J1517-2422, J1625-2527   \\
  &  Oph 1-10                 &  2022-04-09 08:03:   &  C43-2  &  15.1 - 313.7   &     41&   77.9&    0.8&  J1517-2422, J1625-2527   \\
  &  Oph 1-10                 &  2022-07-05 05:14:   &  C43-5  &  15.1 - 1996.7  &     41&   35.7&    1.5&  J1924-2914, J1700-2610   \\
  &  Oph 1-10                 &  2022-07-19 02:05:   &  C43-6  &  15.3 - 2617.4  &     44&   66.3&    0.9&  J1517-2422, J1700-2610   \\
  &  Oph 1-10                 &  2022-07-22 22:40:   &  C43-6  &  15.3 - 2617.4  &     42&   70.4&    1.3&  J1517-2422, J1700-2610   \\
  &  Oph 1-10                 &  2022-07-29 22:18:   &  C43-6  &  15.1 - 2517.3  &     38&   71.5&    1.2&  J1517-2422, J1700-2610   \\
  &  Oph 1-10                 &  2022-07-30 01:32:   &  C43-6  &  15.1 - 2517.3  &     38&   66.2&    1.1&  J1517-2422, J1700-2610   \\
  &  Oph 1-10                 &  2022-07-31 01:36:   &  C43-5  &  15.1 - 1996.7  &     44&   62.1&    1.0&  J1517-2422, J1700-2610   \\
  &  Oph 1-10                 &  2022-08-01 21:37:   &  C43-5  &  15.1 - 1301.6  &     42&   65.0&    1.1&  J1517-2422, J1700-2610   \\
  &  Oph 1-10                 &  2022-08-02 00:52:   &  C43-5  &  15.1 - 1301.6  &     42&   70.1&    0.6&  J1517-2422, J1700-2610   \\
  &  Oph 1-10                 &  2022-08-03 01:26:   &  C43-5  &  15.1 - 1301.6  &     43&   61.5&    0.9&  J1517-2422, J1700-2610   \\
 Lup CO         &  Lupus 1                  &  2022-03-31 06:11:   &  C43-2  &  14.6 - 330.6   &     45&   69.8&    1.1&  J1454-3747               \\
  &  Lupus 1                  &  2022-04-09 07:14:   &  C43-2  &  15.0 - 313.7   &     44&   77.2&    0.9&  J1454-3747               \\
  &  Lupus 1                  &  2018-09-24 20:09:   &  C43-5  &  15.1 - 1397.8  &     44&   74.1&    1.5&  J1610-3958               \\
  &  Lupus 1                  &  2018-09-29 21:33:   &  C43-5  &  15.1 - 1397.8  &     44&   55.4&    1.2&  J1610-3958               \\
  &  Lupus 2-5, 7-9           &  2022-03-25 06:16:   &  C43-2  &  14.6 - 313.7   &     46&   77.1&    0.2&  J1610-3958               \\
  &  Lupus 2-5, 7-9           &  2022-03-25 07:22:   &  C43-2  &  14.6 - 313.7   &     46&   77.1&    0.2&  J1610-3958               \\
  &  Lupus 2-5, 7-9           &  2022-03-25 07:22:   &  C43-2  &  14.6 - 313.7   &     46&   77.1&    0.2&  J1610-3958               \\
  % &  Lupus 2-5, 7-9           &  2021-12-14
  % 12:54:   &  C43-5  &  15.1 - 1397.4  &     41&   70.6&    &  &\\
  % J1610-3958, J1604-4441\\
  &  Lupus 2-5, 7-9           &  2021-12-15 12:58:   &  C43-5  &  15.1 - 1917.1  &     19&   71.7&    1.3&  J1610-3958 and J1604-4441\\
  &  Lupus 2-5, 7-9           &  2022-06-21 00:58:   &  C43-5  &  15.1 - 1301.6  &     39&   74.1&    1.5&  J1610-3958 and J1604-4441\\
  &  Lupus 2-5, 7-9           &  2022-06-21 02:54:   &  C43-5  &  15.1 - 1301.6  &     37&   68.3&    1.1&  J1610-3958 and J1604-4441\\
  &  Lupus 2-5, 7-9           &  2022-06-29 00:56:   &  C43-5  &  15.1 - 1301.6  &     47&   75.9&    0.4&  J1610-3958 and J1604-4441\\
  &  Lupus 10                 &  2022-03-28 06:29:   &  C43-2  &  14.6 - 313.7   &     46&   63.6&    1.8&  J1610-3958               \\
  &  Lupus 10                 &  2021-12-01 14:05:   &  C43-5  &  15.1 - 2617.6  &     43&   66.0&    1.2&  J1610-3958 and J1604-4228\\
 Lup N$_2$H$^{+}$&  Lupus 1, Lupus 6         &  2019-10-10 21:24    &  C43-3  &  15.1 - 783.5   &     45&   49.8&    1.5&  J1610-3958 and J1924-2914\\
  &  Lupus 1, Lupus 6         &  2019-10-30 17:04    &  C43-3  &  15.1 - 696.9   &     45&   74.3&    1.5&  J1427-4206 and J1610-3958\\
  &  Lupus 1, Lupus 6         &  2019-10-30 20:30    &  C43-3  &  15.1 - 696.9   &     45&   44.9&    1.5&  J1610-3958 and J1924-2914\\
  &  Lupus 1, Lupus 6         &  2019-11-07 14:50    &  C43-3  &  15.1 - 500.2   &     45&   62.1&    1.5&  J1427-4206 and J1610-3958\\
  &  Lupus 1, Lupus 6         &  2019-11-07 16:18    &  C43-3  &  15.1 - 500.2   &     45&   73.4&    1.5&  J1427-4206 and J1610-3958\\
  &  Lupus 2-5, 7-10          &  2022-04-13 9:01     &  C43-3  &  15.1 - 500.2   &     46&   66.7&    0.3&  J1517-2422 and J1610-3958\\
  &  Lupus 2-5, 7-10          &  2022-04-15 7:39     &  C43-3  &  15.1 - 500.2   &     43&   76.2&    0.5&  J1427-4206 and J1610-3958\\
  &  Lupus 2-5, 7-10          &  2022-04-15 9:27     &  C43-3  &  15.1 - 479.1   &     46&   60.5&    0.5&  J1517-2422 and J1610-3958\\
  &  Lupus 2-5, 7-10          &  2022-04-16 5:49     &  C43-3  &  15.1 - 500.2   &     48&   66.2&    0.5&  J1517-2422 and J1610-3958\\
  &  Lupus 2-5, 7-10          &  2022-04-16 7:07     &  C43-3  &  15.1 - 500.2   &     48&   76.2&    0.5&  J1427-4206 and J1610-3958\\
  &  Lupus 2-5, 7-10          &  2022-04-16 8:26     &  C43-3  &  15.1 - 500.2   &     48&   70.6&    0.5&  J1517-2422 and J1610-3958\\
 Upp CO         &  UppSco 2, UppSco 3       &  2022-07-03 0:08:57  &   &   &   &   &   &   \\
 Upp N$_2$H$^{+}$&  UppSco 9, UppSco 10      &  2016 March 9:35:00  &  C43-2  &  15.2 - 460     &     41&   78.3&    1.4&  J1517-2422, J1626-2951, J1733-1304 and Titan\\
  &  UppSco 9, UppSco 10      &  2016 March 8:34:00  &  C43-2  &  15.1 - 460     &     40&   72.1&    1.4&  J1517-2422, J1553-2422, J1733-1304 and Titan\\
  &  UppSco 9, UppSco 10      &  2016 March 11:58:00 &  C43-2  &  15.1 - 460     &     39&   48.7&    1.4&  J1517-2422, J1553-2422, J1733-1304 and Titan\\
  &  UppSco 9, UppSco 10      &  2016 March 11:39:00 &  C43-2  &  15.1 - 460     &     38&   52.2&    1.4&  J1517-2422, J1553-2422, J1733-1304 and Titan\\
  &  UppSco 1                 &  2022-04-12 4:32     &  C43-3  &  15.1 - 455.5   &     42&   59.4&    0.6&  J1517-2422 and J1626-2951\\
  &  UppSco 1                 &  2022-04-12 5:34     &  C43-3  &  15.1 - 455.5   &     42&   72.5&    0.6&  J1517-2422 and J1626-2951\\
  &  UppSco 2-8               &  2022-04-17 5:14     &  C43-3  &  15.1 - 500.2   &     46&   75.1&    0.3&  J1517-2422 and J1553-2422\\
  &  UppSco 2-8               &  2022-04-22 8:51     &  C43-3  &  15.1 - 500.2   &     44&   50.1&    0.4&  J1625-2527 and J1924-2914\\
  &  UppSco 2-8               &  2022-04-23 4:53     &  C43-3  &  15.1 - 500.2   &     46&   75.7&    0.5&  J1517-2422 and J1553-2422\\
  &  UppSco 2-8               &  2022-04-23 7:37     &  C43-3  &  15.1 - 500.2   &     46&   66.5&    0.7&  J1517-2422 and J1553-2422\\
  &  UppSco 2-8               &  2022-04-23 8:57     &  C43-3  &  15.1 - 500.2   &     46&   47.7&    0.8&  J1625-2527 and J1924-2914\\
  &  UppSco 2-8               &  2022-04-24 6:55     &  C43-3  &  15.1 - 500.2   &     47&   75.2&    0.4&  J1517-2422 and J1553-2422\\
  &  UppSco 2-8               &  2022-04-24 8:15     &  C43-3  &  15.1 - 500.2   &     47&   56.9&    0.4&  J1517-2422 and J1553-2422\\
  &  UppSco 2-8               &  2022-04-25 8:23     &  C43-3  &  15.1 - 500.2   &     48&   53.8&    0.4&  J1625-2527 and J1924-2914\\
  &  UppSco 2-8               &  2022-04-26 6:54     &  C43-3  &  15.1 - 500.2   &     43&   73.7&    0.6&  J1517-2422 and J1553-2422\\
  &  UppSco 2-8               &  2022-04-26 8:16     &  C43-3  &  15.1 - 500.2   &     43&   55.0&    0.5&  J1517-2422 and J1625-2527\\
  &  UppSco 2-8               &  2022-04-27 7:06     &  C43-3  &  15.1 - 500.2   &     45&   70.0&    1.0&  J1517-2422 and J1553-2422\\
\enddata
\tablecomments{Col.~(1) Target name. Col.~(2) \todo{no UpperSco CO setup yet, separate AGE-PRO from archival setups}}
% \tablenotetext{a}{HT Lup (Sz 68) and AS 205 (V866 Sco) are triple systems.  See \citet{troncoso18} for details.}
% \tablenotetext{b}{The MY Lup disk is inclined and flared enough that it likely extincts the host: the $L_\ast$ and $t_\ast$ estimates may be too faint and old, respectively.}
% \tablerefs{In Col.~(11), the references for the quoted SpT, \{$T_{\rm eff}$, $L_\ast$\}, and accretion luminosity measurements, respectively: 1 = \citet{alcala17}, 2 = \citet{fairlamb15}, 3 = \citet{luhman12}, 4 = \citet{barenfeld16}, 5 = \citet{rigliaco15}, 6 = \citet{salyk13}, 7 = \citet{luhman99b}, 8 = \citet{andrews10b}, 9 = \citet{natta06}, 10 = \citet{andrews09}, 11 = \citet{wilking05}, 12 = \citet{muzerolle98}, 13 = \citet{bouvier92}, 14 = \citet{eisner05}, 15 = \citet{hbc88}.}
\end{deluxetable*}

==> star_table.tex <==
\begin{deluxetable*}{lcccccccccc}
\tabletypesize{\scriptsize}
\tablecaption{AGE-PRO Sample: Host Star Properties \label{table:stars}}
\tablewidth{0pt}
\tablehead{
\colhead{Index} & \colhead{Source Name} & \colhead{RA} & \colhead{Dec}  & \colhead{$d$} & 
\colhead{$T_{\rm eff}$} & \colhead{$L_\ast$} & \colhead{Av} & \colhead{$M_\ast$} & \colhead{$\log{\dot{M}_\ast}$} & \colhead{Refs.} 
\\
\colhead{} & \colhead{} &  \colhead{(h m s)} & \colhead{(d m s)} & \colhead{(pc)} & 
\colhead{(K)} & \colhead{($L_\odot$)} & \colhead{($M_\odot$)} & 
\colhead{(yr)} & \colhead{$M_\odot \, {\rm yr}^{-1}$} & \colhead{}
}
\decimalcolnumbers
\startdata
 Oph 1     &  SSTc2dJ162623.6-242439   &  16:26:23.600&  -24:24:39.000 &  139.0&  4020  &  0.51 &  \nodata  &  0.69 &  -8.500    & \\
 Oph 2     &  SSTc2dJ162703.6-242005   &  16:27:03.600&  -24:20:05.000 &  139.0&  3698  &  \nodata  &  \nodata  &  \nodata  &  \nodata       & \\
 Oph 3     &  SSTc2dJ162719.2-242844   &  16:27:19.200&  -24:28:44.000 &  139.0&  4074  &  \nodata  &  \nodata  &  \nodata  &  \nodata       & \\
 Oph 4     &  SSTc2dJ162728.4-242721   &  16:27:28.400&  -24:27:21.000 &  139.0&  4020  &  1.40 &  \nodata  &  0.55 &  -7.980    & \\
 Oph 5     &  SSTc2dJ162737.2-244237   &  16:27:37.200&  -24:42:38.000 &  139.0&  3890  &  \nodata  &  \nodata  &  \nodata  &  \nodata       & \\
 Oph 6     &  SSTc2dJ162738.9-244020   &  16:27:38.900&  -24:40:20.000 &  139.0&  3485  &  0.06 &  \nodata  &  0.39 &  -8.953    & \\
 Oph 7     &  SSTc2dJ163135.6-240129   &  16:31:35.600&  -24:01:29.000 &  139.0&  4227  &  \nodata  &  \nodata  &  \nodata  &  \nodata       & \\
 Oph 8     &  2MASSJ16230544-2302566   &  16:23:05.400&  -23:02:57.000 &  139.0&  3681  &  \nodata  &  \nodata  &  \nodata  &  \nodata       & \\
 Oph 9     &  SSTc2dJ162627.5-244153   &  16:26:27.500&  -24:41:54.000 &  139.0&  3532  &  \nodata  &  \nodata  &  \nodata  &  \nodata       & \\
 Oph 10    &  SSTc2dJ162718.4-243915   &  16:27:18.400&  -24:39:15.000 &  139.0&  3837  &  \nodata  &  \nodata  &  \nodata  &  \nodata       & \\
 Lupus 1   &  Sz 65                    &  15:39:27.753&  -34:46:17.577 &  153.5&  4020  &  0.87 &  0.6  &  0.61 &  -9.480    & \\
 Lupus 2   &  Sz 71                    &  15:46:44.709&  -34:30:36.054 &  155.2&  3640  &  0.33 &  0.5  &  0.41 &  -9.033    & \\
 Lupus 3   &  2MASSJ16124373-3815031   &  16:12:43.736&  -38:15:03.471 &  159.8&  3720  &  0.39 &  0.8  &  0.47 &  -9.084    & \\
 Lupus 4   &  Sz 72                    &  15:47:50.608&  -35:28:35.779 &  156.7&  3560  &  0.27 &  0.8  &  0.37 &  -8.601    & \\
 Lupus 5   &  Sz 77                    &  15:51:46.941&  -35:56:44.531 &  155.2&  4020  &  0.59 &  0.0  &  0.67 &  -8.690    & \\
 Lupus 6   &  2MASSJ16085324-3914401   &  16:08:53.227&  -39:14:40.553 &  163.0&  3410  &  0.20 &  1.9  &  0.29 &  -10.030   & \\
 Lupus 7   &  Sz 131                   &  16:00:49.414&  -41:30:04.263 &  160.6&  3410  &  0.15 &  0.0  &  0.30 &  -9.171    & \\
 Lupus 8   &  Sz 66                    &  15:39:28.264&  -34:46:18.450 &  155.9&  3410  &  0.22 &  1.0  &  0.29 &  -8.508    & \\
 Lupus 9   &  Sz 95                    &  16:07:52.293&  -38:58:06.446 &  160.5&  3410  &  0.27 &  0.8  &  0.29 &  -9.381    & \\
 Lupus 10  &  V1094 Sco                &  16:08:36.160&  -39:23:02.879 &  158.0&  4205  &  1.15 &  1.7  &  0.83 &  -8.040    & \\
 UppSco 1  &  2MASSJ16120668-3010270   &  16:12:06.68 &  -30:10:27.0   &  132.0&  3776  &  0.25 &  \nodata  &  \nodata  &  \nodata       & \\
 UppSco 2  &  2MASSJ16054540-2023088   &  16:05:45.403&  -20:23:08.815 &  138.7&  3085  &  0.09 &  0.6  &  0.15 &  -9.358    & \\
 UppSco 3  &  2MASSJ16020757-2257467   &  16:02:07.575&  -22:57:46.778 &  140.7&  3560  &  0.08 &  0.4  &  0.45 &  -10.980   & \\
 UppSco 4  &  2MASSJ16111742-1918285   &  16:11:17.42 &  -19:18:28.5   &  137.0&  3811  &  0.32 &  \nodata  &  \nodata  &  \nodata       & \\
 UppSco 5  &  2MASSJ16145026-2332397   &  16:14:50.26 &  -23:32:39.7   &  144.0&  3412  &  0.09 &  \nodata  &  \nodata  &  \nodata       & \\
 UppSco 6  &  2MASSJ16163345-2521505   &  16:16:33.455&  -25:21:50.566 &  159.4&  3776  &  0.17 &  1.1  &  0.51 &  \nodata       & \\
 UppSco 7  &  2MASSJ16202863-2442087   &  16:20:28.63 &  -24:42:08.7   &  153.0&  3556  &  0.18 &  \nodata  &  \nodata  &  \nodata       & \\
 UppSco 8  &  2MASSJ16221532-2511349   &  16:22:15.32 &  -25:11:34.9   &  139.0&  3412  &  0.10 &  \nodata  &  \nodata  &  \nodata       & \\
 UppSco 9  &  2MASSJ16082324-1930009   &  16:08:23.246&  -19:30:00.932 &  137.8&  3900  &  0.32 &  1.1  &  0.65 &  -9.138    & \\
 UppSco 10 &  2MASSJ16090075-1908526   &  16:09:00.759&  -19:08:52.616 &  137.4&  3900  &  0.32 &  1.0  &  0.65 &  -8.808    & \\
 \enddata
\tablecomments{Col.~(1) Target name. Col.~(2) \todo{add SpT, Class}}
% \tablenotetext{a}{HT Lup (Sz 68) and AS 205 (V866 Sco) are triple systems.  See \citet{troncoso18} for details.}
% \tablenotetext{b}{The MY Lup disk is inclined and flared enough that it likely extincts the host: the $L_\ast$ and $t_\ast$ estimates may be too faint and old, respectively.}
% \tablerefs{In Col.~(11), the references for the quoted SpT, \{$T_{\rm eff}$, $L_\ast$\}, and accretion luminosity measurements, respectively: 1 = \citet{alcala17}, 2 = \citet{fairlamb15}, 3 = \citet{luhman12}, 4 = \citet{barenfeld16}, 5 = \citet{rigliaco15}, 6 = \citet{salyk13}, 7 = \citet{luhman99b}, 8 = \citet{andrews10b}, 9 = \citet{natta06}, 10 = \citet{andrews09}, 11 = \citet{wilking05}, 12 = \citet{muzerolle98}, 13 = \citet{bouvier92}, 14 = \citet{eisner05}, 15 = \citet{hbc88}.}
\end{deluxetable*}
